Product Graph Learning from Multi-attribute Graph Signals with Inter-layer Coupling

This paper considers learning a product graph from multi-attribute graph signals. Our work is motivated by the widespread presence of multilayer networks that feature interactions within and across graph layers. Focusing on a product graph setting with homogeneous layers, we propose a bivariate polynomial graph filter model. We then consider the topology inference problems thru adapting existing spectral methods. We propose two solutions for the required spectral estimation step: a simplified solution via unfolding the multi-attribute data into matrices, and an exact solution via nearest Kronecker product decomposition (NKD). Interestingly, we show that strong inter-layer coupling can degrade the performance of the unfolding solution while the NKD solution is robust to inter-layer coupling effects. Numerical experiments show efficacy of our methods.

==> fig/simulation/centrality/cen_m.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=80,
xmax=2000,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={m},
ymin=0,
ymax=0.8,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{centra error rate N}_\text{g}\text{=60 N}_\text{c}\text{=3  kron product}$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
80	0.706\\
100	0.704\\
200	0.054\\
500	0.002\\
1000	0\\
2000	0\\
};
\addlegendentry{our opi}

\addplot [color=mycolor2, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
80	0.678\\
100	0.692\\
200	0.65\\
500	0.658\\
1000	0.624\\
2000	0.602\\
};
\addlegendentry{benchmark opi}

\addplot [color=mycolor3, mark=asterisk, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
80	0\\
100	0\\
200	0\\
500	0\\
1000	0\\
2000	0\\
};
\addlegendentry{our exp}

\addplot [color=mycolor4, mark=o, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
80	0\\
100	0\\
200	0\\
500	0\\
1000	0\\
2000	0\\
};
\addlegendentry{benchmark exp}

\end{axis}
\end{tikzpicture}%

==> fig/simulation/centrality/cen_m_new.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=100,
xmax=1000000,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={m},
ymin=0,
ymax=0.9,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{centra error rate N}_\text{g}\text{=80 N}_\text{c}\text{=3}$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
100	0.878000000000001\\
200	0.694\\
500	0\\
1000	0\\
2000	0\\
50000	0\\
500000	0\\
};
\addlegendentry{Algo1-nonsep}

\addplot [color=mycolor2, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
100	0.838\\
200	0.75\\
500	0.559\\
1000	0.362\\
2000	0.217\\
50000	0.027\\
500000	0.011\\
};
\addlegendentry{Algo2-nonsep}

\addplot [color=mycolor3, mark=asterisk, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
100	0\\
200	0\\
500	0\\
1000	0\\
2000	0\\
50000	0\\
500000	0\\
};
\addlegendentry{Algo1-sep}

\addplot [color=mycolor4, mark=o, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
100	0\\
200	0\\
500	0\\
1000	0\\
2000	0\\
50000	0\\
500000	0\\
};
\addlegendentry{Algo2-sep}

\end{axis}
\end{tikzpicture}%

==> fig/simulation/centrality/cen_n.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmin=20,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{N}_\text{g}$},
ymin=0,
ymax=0.9,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{centra error ratem=400 N}_\text{c}\text{=3  kron product}$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
20	0\\
30	0.001\\
40	0\\
50	0.001\\
60	0.002\\
80	0.001\\
100	0.008\\
};
\addlegendentry{our opi}

\addplot [color=mycolor2, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
20	0.328\\
30	0.488\\
40	0.578\\
50	0.674\\
60	0.726\\
80	0.781\\
100	0.839\\
};
\addlegendentry{benchmark opi}

\addplot [color=mycolor3, mark=asterisk, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
20	0\\
30	0\\
40	0\\
50	0\\
60	0\\
80	0\\
100	0\\
};
\addlegendentry{our exp}

\addplot [color=mycolor4, mark=o, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
20	0\\
30	0\\
40	0\\
50	0\\
60	0\\
80	0\\
100	0\\
};
\addlegendentry{benchmark exp}

\end{axis}
\end{tikzpicture}%

==> fig/simulation/centrality/cen_n_new.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=20,
xmax=100,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{N}_\text{g}$},
ymin=0,
ymax=0.8,
ylabel style={font=\color{white!15!black}},
ylabel={$\text{centra error rate m=400 N}_\text{c}\text{=3}$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
20	0\\
30	0.002\\
40	0.001\\
50	0.001\\
60	0.001\\
80	0.003\\
100	0.014\\
};
\addlegendentry{Algo1-nonsep}

\addplot [color=mycolor2, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
20	0.372\\
30	0.477\\
40	0.505\\
50	0.563\\
60	0.565\\
80	0.62\\
100	0.726\\
};
\addlegendentry{Algo2-nonsep}

\addplot [color=mycolor3, mark=asterisk, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
20	0\\
30	0.001\\
40	0\\
50	0\\
60	0\\
80	0\\
100	0\\
};
\addlegendentry{Algo1-sep}

\addplot [color=mycolor4, mark=o, mark options={solid, mycolor4}]
  table[row sep=crcr]{%
20	0\\
30	0.001\\
40	0\\
50	0\\
60	0\\
80	0\\
100	0\\
};
\addlegendentry{Algo2-sep}

\end{axis}
\end{tikzpicture}%

==> fig/simulation/pgl/pgl_compare.tex <==
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{groupplot}[group style={group name=myplot,group size=2 by 1}]
\nextgroupplot[%
% width=6.028in,
% height=4.754in,
% at={(1.011in,0.642in)},
% scale only axis,
xmin=2,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{N}_\text{g}$},
ymin=0.6,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={F score lowpass},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, mark=o, mark options={solid, blue}]
  table[row sep=crcr]{%
3	1\\
5	0.916650874495302\\
6	0.866806311520997\\
8	0.863262322140714\\
10	0.837556688682468\\
15	0.806452746723952\\
20	0.810660284105317\\
};
\addlegendentry{kron(a)}

\addplot [color=black, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
3	0.714153846153845\\
5	0.637974883686193\\
6	0.661170442126589\\
8	0.657221354266205\\
10	0.663678174069664\\
15	0.667965932481698\\
20	0.644134031249328\\
};
\addlegendentry{Pgl(a)}

\addplot [color=mycolor1, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
3	1\\
5	0.914540786870508\\
6	0.870083053333967\\
8	0.850489232968309\\
10	0.832614148670264\\
15	0.804516718697328\\
20	0.806204146382958\\
};
\addlegendentry{sep(a)}

\addplot [color=blue, dashed, mark=asterisk, mark options={solid, blue}]
  table[row sep=crcr]{%
3	1\\
5	0.937350880419515\\
6	0.904926102568663\\
8	0.890305098761756\\
10	0.866041001901506\\
15	0.845331647926457\\
20	0.826111883984793\\
};
\addlegendentry{kron(b)}

\addplot [color=black, dashed, mark=asterisk, mark options={solid, black}]
  table[row sep=crcr]{%
3	0.849999999999999\\
5	0.828273246332192\\
6	0.817851186425601\\
8	0.826550171320395\\
10	0.816742417079985\\
15	0.827390178002234\\
20	0.822287186256717\\
};
\addlegendentry{Pgl(b)}

\addplot [color=mycolor1, dashed, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
3	1\\
5	0.940370575064484\\
6	0.920827724470592\\
8	0.886507770914752\\
10	0.871824770530038\\
15	0.849854479568081\\
20	0.828605037397594\\
};
\addlegendentry{sep(b)}



\nextgroupplot[%
% width=6.028in,
% height=4.754in,
% at={(1.011in,0.642in)},
% scale only axis,
xmin=2,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{N}_\text{g}$},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={F score highpass},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, mark=o, mark options={solid, blue}]
  table[row sep=crcr]{%
3	1\\
5	0.932539361223572\\
6	0.865493441590893\\
8	0.865049266183985\\
10	0.821405066723681\\
15	0.799781500951581\\
20	0.822791776427101\\
};
\addlegendentry{kron(a)}

\addplot [color=black, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
3	0.001\\
5	0.001\\
6	0.001\\
8	0.00283679245283019\\
10	0.001\\
15	0.001\\
20	0.001\\
};
\addlegendentry{Pgl(a)}

\addplot [color=mycolor1, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
3	1\\
5	0.909331501831502\\
6	0.858247019951826\\
8	0.871640914066062\\
10	0.821034423564022\\
15	0.80121924891759\\
20	0.821849387151235\\
};
\addlegendentry{sep(a)}

\addplot [color=blue, dashed, mark=asterisk, mark options={solid, blue}]
  table[row sep=crcr]{%
3	1\\
5	0.898232455738976\\
6	0.894348850801756\\
8	0.872500749485652\\
10	0.86237102776343\\
15	0.846541584155227\\
20	0.83445049135993\\
};
\addlegendentry{kron(b)}

\addplot [color=black, dashed, mark=asterisk, mark options={solid, black}]
  table[row sep=crcr]{%
3	0.001\\
5	0.001\\
6	0.001\\
8	0.0139452455590387\\
10	0.001\\
15	0.001\\
20	0.001\\
};
\addlegendentry{Pgl(b)}

\addplot [color=mycolor1, dashed, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
3	1\\
5	0.955780419524975\\
6	0.928081386125029\\
8	0.879516520254048\\
10	0.877260593245003\\
15	0.858088559046601\\
20	0.820697940149449\\
};
\addlegendentry{sep(b)}

\end{groupplot}
\end{tikzpicture}%

==> fig/simulation/pgl/topo_ng_tau_pro100_compa.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmin=2,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{N}_\text{g}$},
ymin=0.6,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={F score our signal model},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, mark=o, mark options={solid, blue}]
  table[row sep=crcr]{%
3	1\\
5	0.916650874495302\\
6	0.866806311520997\\
8	0.863262322140714\\
10	0.837556688682468\\
15	0.806452746723952\\
20	0.810660284105317\\
};
\addlegendentry{kron(a)}

\addplot [color=black, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
3	0.714153846153845\\
5	0.637974883686193\\
6	0.661170442126589\\
8	0.657221354266205\\
10	0.663678174069664\\
15	0.667965932481698\\
20	0.644134031249328\\
};
\addlegendentry{Pgl(a)}

\addplot [color=mycolor1, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
3	1\\
5	0.914540786870508\\
6	0.870083053333967\\
8	0.850489232968309\\
10	0.832614148670264\\
15	0.804516718697328\\
20	0.806204146382958\\
};
\addlegendentry{sep(a)}

\addplot [color=blue, dashed, mark=asterisk, mark options={solid, blue}]
  table[row sep=crcr]{%
3	1\\
5	0.937350880419515\\
6	0.904926102568663\\
8	0.890305098761756\\
10	0.866041001901506\\
15	0.845331647926457\\
20	0.826111883984793\\
};
\addlegendentry{kron(b)}

\addplot [color=black, dashed, mark=asterisk, mark options={solid, black}]
  table[row sep=crcr]{%
3	0.849999999999999\\
5	0.828273246332192\\
6	0.817851186425601\\
8	0.826550171320395\\
10	0.816742417079985\\
15	0.827390178002234\\
20	0.822287186256717\\
};
\addlegendentry{Pgl(b)}

\addplot [color=mycolor1, dashed, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
3	1\\
5	0.940370575064484\\
6	0.920827724470592\\
8	0.886507770914752\\
10	0.871824770530038\\
15	0.849854479568081\\
20	0.828605037397594\\
};
\addlegendentry{sep(b)}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%

==> fig/simulation/pgl/topo_ng_tau_pro100_compa_high.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmin=2,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={$\text{N}_\text{g}$},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={F score our signal model high},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, mark=o, mark options={solid, blue}]
  table[row sep=crcr]{%
3	1\\
5	0.932539361223572\\
6	0.865493441590893\\
8	0.865049266183985\\
10	0.821405066723681\\
15	0.799781500951581\\
20	0.822791776427101\\
};
\addlegendentry{kron(a)}

\addplot [color=black, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
3	0.001\\
5	0.001\\
6	0.001\\
8	0.00283679245283019\\
10	0.001\\
15	0.001\\
20	0.001\\
};
\addlegendentry{Pgl(a)}

\addplot [color=mycolor1, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
3	1\\
5	0.909331501831502\\
6	0.858247019951826\\
8	0.871640914066062\\
10	0.821034423564022\\
15	0.80121924891759\\
20	0.821849387151235\\
};
\addlegendentry{sep(a)}

\addplot [color=blue, dashed, mark=asterisk, mark options={solid, blue}]
  table[row sep=crcr]{%
3	1\\
5	0.898232455738976\\
6	0.894348850801756\\
8	0.872500749485652\\
10	0.86237102776343\\
15	0.846541584155227\\
20	0.83445049135993\\
};
\addlegendentry{kron(b)}

\addplot [color=black, dashed, mark=asterisk, mark options={solid, black}]
  table[row sep=crcr]{%
3	0.001\\
5	0.001\\
6	0.001\\
8	0.0139452455590387\\
10	0.001\\
15	0.001\\
20	0.001\\
};
\addlegendentry{Pgl(b)}

\addplot [color=mycolor1, dashed, mark=asterisk, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
3	1\\
5	0.955780419524975\\
6	0.928081386125029\\
8	0.879516520254048\\
10	0.877260593245003\\
15	0.858088559046601\\
20	0.820697940149449\\
};
\addlegendentry{sep(b)}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%
